EASYTOOL: Enhancing LLM-based Agents with Concise Tool Instruction

To address intricate real-world tasks, there has been a rising interest in tool utilization in applications of large language models (LLMs). To develop LLM-based agents, it usually requires LLMs to understand many tool functions from different tool documentation. But these documentations could be diverse, redundant or incomplete, which immensely affects the capability of LLMs in using tools. To solve this, we introduce EASYTOOL, a framework transforming diverse and lengthy tool documentation into a unified and concise tool instruction for easier tool usage. EasyTool purifies essential information from extensive tool documentation of different sources, and elaborates a unified interface (i.e., tool instruction) to offer standardized tool descriptions and functionalities for LLM-based agents. Extensive experiments on multiple different tasks demonstrate that EasyTool can significantly reduce token consumption and improve the performance of tool utilization in real-world scenarios. Our code will be available at \url{https://github.com/microsoft/JARVIS/} in the future.

==> list/020instruction_generation.tex <==

\lstset{
    backgroundcolor=\color[RGB]{245,245,244},
    breaklines=true,
    breakindent=0pt,
    basicstyle=\ttfamily\small,
    emphstyle={\bfseries\color{NavyBlue}}
}\begin{lstlisting}[caption={Instruction templates for ChatGPT to generate the tool instruction for FuncQA},label=lst:instruction_generation]
Your task is to generate a tool instruction for the tool given the function of the tool.
The tool instruction consists of two parts: tool description and tool function guidelines.

The tool description only contains the purposes of the tool without other irrelevant information. Here is an example:
'add_' returns the sum of all the arguments passed to it, normalized to 2 decimal places.

The tool function guidelines introduce the parameters with examples that contain the scenario adopting the parameters. Here is an example:
"Usage":
{
    "required_parameters":[
        {
               "name":"input",
               "type":"List"
        }
    ],
         "Example":{
            "Scenario":"if you want to add 2 to 1.",
            "Parameters":{
               "input":[2,1]
        }
    }
}

You should first generate the tool description and then give the tool function guidelines. You must only output in a parsible JSON format. Two example outputs look like:
{"tool_description": XX, "Usage": XX}

This is the tool name: {tool_name}
This is the function of tool: {tool_function}
Output: 
\end{lstlisting}

==> list/040LLMLingua.tex <==
\lstset{
    backgroundcolor=\color[RGB]{245,245,244},
    breaklines=true,
    breakindent=0pt,
    basicstyle=\ttfamily\small,
    emph={Prompt,-,1,2,3},
    emphstyle={\bfseries\color{NavyBlue}}
}\begin{lstlisting}[caption={The original tool documentation and tool instruction compressed by LLMLingua},label=lst:LLMLingua]
{
    "product_id": "api_082f18b5-9054-4488-809f-a40126e2ccfa",
    "tool_description": "Welcome to our e-commerce API! Our API is designed to make it easy for you to build and manage your online store and also build projects you can show on your porfolio. With our API, you can create products, manage orders, track shipments, and more. Our API is built on modern technologies and is easy to integrate with your existing systems.  Our API provides a secure and reliable platform for your e-commerce needs. You can trust us to keep your data safe and secure. We also provide a range of ...",
    "home_url": "https://rapidapi.com/JesutoniAderibigbe/api/cartify/",
    "name": "Cartify",
    "title": "Cartify",
    "pricing": "FREE",
    "tool_name": "Cartify",
    "host": "cartify.p.rapidapi.com",
    "api_list": [
        {
            "name": "getOrders",
            "url": "https://cartify.p.rapidapi.com/users/api/v1/admin/orders",
            "description": "The endpoint retrieves all orders.\n\nSet the authorization to \"Bearer admin\" to authorize that the admin can check and confirm all orders.\n\nYou should get a JSON object with the following attributes;\nid (integer): The unique identifier for the order.\ndeliveryDate(Date): The date that the user wants the order to be delivered\ndestination(String): Location\nAlongside with the user who ordered the product",
            "method": "GET",
            "required_parameters": [],
            "optional_parameters": [],
            "code": "import requests\n\nurl = \"https://cartify.p.rapidapi.com/users/api/v1/admin/orders\"\n\nheaders = {\n            \"X-RapidAPI-Key\": \"SIGN-UP-FOR-KEY\",\n            \"X-RapidAPI-Host\": \"cartify.p.rapidapi.com\"\n        }\n\nresponse = requests.get(url, headers=headers)\nprint(response.json())\n",
            "convert_code": "import requests\n\nurl = \"https://cartify.p.rapidapi.com/users/api/v1/admin/orders\"\n\nheaders = {\n            \"X-RapidAPI-Key\": \"SIGN-UP-FOR-KEY\",\n            \"X-RapidAPI-Host\": \"cartify.p.rapidapi.com\"\n        }\n\nresponse = requests.get(url, headers=headers)\nprint(response.json())\n"
        },
        {
            "name": "getProducts",
            "url": "https://cartify.p.rapidapi.com/products",
            "description": "This endpoint gets all products in the database.\n\nA list of products in the store, with the following attributes:\n\nid (integer): The unique identifier for the product.\ntitle (string): The name of the product.\ncategory (string): A description of the product.\nprice (number): The price of the product.\nimage_url (string): A URL to an image of the product.",
            "method": "GET",
            "required_parameters": [],
            "optional_parameters": [],
            "code": "import requests\n\nurl = \"https://cartify.p.rapidapi.com/products\"\n\nheaders = {\n            \"X-RapidAPI-Key\": \"SIGN-UP-FOR-KEY\",\n            \"X-RapidAPI-Host\": \"cartify.p.rapidapi.com\"\n        }\n\nresponse = requests.get(url, headers=headers)\nprint(response.json())\n",
            "convert_code": "import requests\n\nurl = \"https://cartify.p.rapidapi.com/products\"\n\nheaders = {\n            \"X-RapidAPI-Key\": \"SIGN-UP-FOR-KEY\",\n            \"X-RapidAPI-Host\": \"cartify.p.rapidapi.com\"\n        }\n\nresponse = requests.get(url, headers=headers)\nprint(response.json())\n",
            "statuscode": 200,
            "schema": {}
        }
    ],
    "standardized_name": "cartify"
}
\end{lstlisting}
